Distributed Experiment Design and Control for Multi-agent Systems with Gaussian Processes

This paper focuses on distributed learning-based control of decentralized multi-agent systems where the agents' dynamics are modeled by Gaussian Processes (GPs). Two fundamental problems are considered: the optimal design of experiment for concurrent learning of the agents' GP models, and the distributed coordination given the learned models. Using a Distributed Model Predictive Control (DMPC) approach, the two problems are formulated as distributed optimization problems, where each agent's sub-problem includes both local and shared objectives and constraints. To solve the resulting complex and non-convex DMPC problems efficiently, we develop an algorithm called Alternating Direction Method of Multipliers with Convexification (ADMM-C) that combines a distributed ADMM algorithm and a Sequential Convexification method. The computational efficiency of our proposed method comes from the facts that the computation for solving the DMPC problem is distributed to all agents and that efficient convex optimization solvers are used at the agents for solving the convexified sub-problems. We also prove that, under some technical assumptions, the ADMM-C algorithm converges to a stationary point of the penalized optimization problem. The effectiveness of our approach is demonstrated in numerical simulations of a multi-vehicle formation control example.

==> lingp-mpc.tex <==

Our previous work \cite{nghiem2019linearized,nghiem2019fast} proposed the \emph{linearized Gaussian Process} (\linGP) concept and developed the \linGP based Sequential Convex Programming (\linGP-SCP) method for solving non-convex GP-MPC problems, which we will summarize and apply to the GP-DMPC problem~\eqref{eq:gpdmpc} in this section. 

\subsection{Linearized Gaussian Processes}
\label{sec:lingp-mpc:lingp}

The \linGP approach approximates a GP $\GPModel_f$ of a nonlinear function $f(x): \RR^{n} \to \RR$ in a small neighborhood of a nominal input $x$ by linearizing the \emph{latent function} $f$ around $x$ and forming a stochastic process, denoted by $\linGPModel{f}{x}$, of the linearized function $\tilde{f}_x$ of $f$ at $x$.
While \linGP seems similar to linearizing the predicted mean and variance equations of $\GPModel_f$ at $x$, it is fundamentally different in the sense that it linearizes the underlying function $f$ directly, resulting in a valid stochastic process $\linGPModel{f}{x}$ on which predictions are made, rather than linearizing certain statistics of the prediction on the original GP.
Indeed, $\linGPModel{f}{x}$ is also a GP, as a distribution over linear functions $\tilde{f}_x$, whose mean is a linear function of the input residual $\Delta x$ and whose variance is a convex quadratic function of $\Delta x$. 



Specifically, consider the linearization of the latent function $f$ around $x$: $f(x + \Delta x) \approx \tilde{f}_{x}(\Delta x) = f(x) + \Delta x^{T} \nabla_{x} f(x)$.
Here, we assume that $f$ is differentiable at $x$ and denote its gradient by $g \equiv \nabla_{x} f$.
Define $\hat{x} = [1, \Delta x^{T}]^{T}$ and $\hat{f}(x) = [f(x), g^{T}(x)]^{T}$.
It is shown in \cite{nghiem2019linearized} that $\hat{f}$ is a multivariate GP derived from $\GPModel_f$, therefore $\tilde{f}_{x}$ is a GP and $\tilde{f}_{x}(\Delta x)$ has a Gaussian distribution with mean $\linGPmean{f}{x}(\Delta x) = \hat{m}_x^{T} \hat{x}$ and variance $\linGPvar{f}{x}(\Delta x) = \hat{x}^{T} \hat{V}_x \hat{x}$, where vector $\hat{m}_x$ and positive semi-definite (PSD) matrix $\hat{V}_x$ are the mean vector and covariance matrix of $\hat{f}$:
\begin{gather}
  \label{eq:derivative-distribution}
  \hat{m}_x =
  \begin{bsmallmatrix}
    \mathrm{k}_{x,X} \\ K^{(1,0)}_{x,X}
  \end{bsmallmatrix}
  \left( K + \sigma_{n}^{2} \IdentityMatrix \right)^{-1} Y \nonumber \\
  \hat{V}_x =
  \left[\begin{smallmatrix}
      \mathrm{k}_{x,x} & K^{(0,1)}_{x,x} \\
      K^{(1,0)}_{x,x} & K^{(1,1)}_{x,x}
    \end{smallmatrix}\right] -
  \begin{bsmallmatrix}
      \mathrm{k}_{x,X} \\ K^{(1,0)}_{x,X}
    \end{bsmallmatrix}
  \scriptstyle\left( K + \sigma_{n}^{2} \IdentityMatrix \right)^{-1}
  \left[\begin{smallmatrix}
      \mathrm{k}_{X,x} & K^{(0,1)}_{X,x}
    \end{smallmatrix}\right]
  \nonumber
\end{gather}
Here, $X = \{x^{(i)}\}_{i = 1,\dots,N}$ and $Y = \{y^{(i)}\}_{i = 1,\dots,N}$ are respectively the set of $N$ observation inputs $x^{(i)}$ and the vector of $N$ corresponding observations $y^{(i)}$ (\ie training data), $\mathrm{k}(x,x')$ is the covariance function of $\GPModel_f$, $K$ is the covariances matrix, $\sigma_n^2$ is the Gaussian noise variance, $\IdentityMatrix$ is an identity matrix of appropriate dimensions,
$K^{(1,0)} = (\nabla_{x} \mathrm{k})$ is the gradient of $\mathrm{k}$ with respect to the first argument, $K^{(0,1)} = (D_{x'} \mathrm{k})$ the Jacobian of $\mathrm{k}$ with respect to the second argument, and $K^{(1,1)}(x,x')$ the matrix such that $K^{(1,1)}_{i,j}(x,x') = \frac{\partial^{2}}{\partial x_{i} \partial x'_{j}} \mathrm{k}(x,x')$.
We also use the convention in \cite{nghiem2019linearized} that when an argument of a scalar function is a collection of arguments, the function application is broadcast along the corresponding dimension; \eg $K(X,X)$ is a $N \times N$ matrix with $K_{i,j}(X,X) = \mathrm{k}(x^{(i)}, x^{(j)})$.
We assume that $\mathrm{k}(\cdot, \cdot)$ is differentiable, which holds for most practical covariance functions \cite{solak2003derivative}.

\subsection{linGP-SCP algorithm for GP-DMPC}
\label{sec:lingp-mpc:lingp-scp}

In \cite{nghiem2019linearized}, a Sequential Convex Programming algorithm \cite{mao2017successive,zilloberVeryLargeScale2004} based on linGP, called linGP-SCP, was developed to solve non-convex GP-MPC problems of a single dynamical system, where each convex subproblem is obtained by replacing the GPs with their linGP approximations around the nominal inputs.
If the GP-DMPC problem~\eqref{eq:gpdmpc} is solved centrally by a global coordinator, the \linGP-SCP algorithm can be applied directly as presented below.

Suppose that at time-step $t$, a feasible nominal solution of \eqref{eq:gpdmpc} is given, for each agent $i$, by $\UUU_{i,t}^{\star} = \{ \mathbf{u}^{\star}_{i,k} \,|\, k \in \III_t \}$ and $\ZZZ_{i,t}^{\star} = \{ \mathbf{z}_{i,k} \,|\, k \in \III_t \}$, that satisfy the constraints of \eqref{eq:gpdmpc}.
The GP models of each agent are simulated over the MPC horizon to obtain the nominal output means $\overbar{\YYY}_{i,t}^{\star} = \{\overbar{\mathbf{y}}_{i,k}^{\star} \,|\, k \in \III_t\}$ and the nominal output variances $\SSS_{i,t}^{\star} = \{\sigma_{i,k}^{\star 2} \,|\, k \in \III_t\}$.
For each agent $i$, consider a small neighborhood of the nominal solution $\mathbf{u}_{i,k} = \mathbf{u}_{i,k}^{\star} + \Delta \mathbf{u}_{i,k}$ and $\mathbf{z}_{i,k} = \mathbf{z}_{i,k}^{\star} + \Delta \mathbf{z}_{i,k}$, where $\Delta \mathbf{u}_{i,k}$ and $\Delta \mathbf{z}_{i,k}$ are collected in $\Delta \UUU_{i,t} = \{ \Delta \mathbf{u}_{i,k} \,|\, k \in \III_t\}$ and $\Delta \ZZZ_{i,t} = \{ \Delta \mathbf{z}_{i,k} \,|\, k \in \III_t\}$ respectively.
This will cause perturbations to the GP regressor $\textbf{x}_{i,k}^{\star}$ as $\Delta \mathbf{x}_{i,k} = \textbf{x}_{i,k} - \textbf{x}_{i,k}^{\star}$ and, consequently, perturbations in the predictive output means and variances of the GPs during the MPC horizon as $\Delta \overbar{\YYY}_{i,t} = \{\Delta \overbar{\mathbf{y}}_{i,k} = \overbar{\mathbf{y}}_{i,k} - \overbar{\mathbf{y}}_{i,k}^{\star} \,|\, k \in \III_t\}$ and $\Delta \SSS_{i,t} = \{\Delta \sigma_{i,k}^2 = \sigma_{i,k}^2 - \sigma_{i,k}^{\star 2} \,|\, k \in \III_t\}$.

We replace the GP models by their \linGP models at each time step $k$ as follows.
Define approximate variables $\tilde{\mathbf{y}}_{i,k}$ of $\overbar{\mathbf{y}}_{i,k}$ and $\tilde{\sigma}_{i,k}^2$ of $\sigma_{i,k}^2$, and collect them for $k \in \III_t$ in $\tilde{\YYY}_{i,t}$ and $\tilde{\SSS}_{i,t}$ respectively.
From \eqref{eq:derivative-distribution}, $\tilde{\mathbf{y}}_{i,k}$ and $\tilde{\sigma}_{i,k}^2$ are respectively linear and convex quadratic in $\hat{\mathbf{x}}_{i,k} = [1, \Delta \mathbf{x}_{i,k}^T]^T$.
With a slight abuse of notations, we will write $\UUU_{i,t} = \UUU_{i,t}^{\star} + \Delta \UUU_{i,t}$ and $\ZZZ_{i,t} = \ZZZ_{i,t}^{\star} + \Delta \ZZZ_{i,t}$. %
All the above notations are also applied to the common concatenated vectors of each agent. 

We now obtain the approximate problem with \linGP, called the \emph{\linGP-DMPC subproblem}, with a trust region radius $\rho$ on the perturbation variables as follows.
\begin{subequations}
  \label{eq:lingpdmpc}
  \begin{align}
    &
      \begin{multlined}
        \underset{\{\Delta \UUU_{i}, \Delta \ZZZ_{i}\}_i}{\text{minimize}} \; 
        \textstyle\sum_{i=1}^M J_i(\tilde{\YYY}_{i}, \tilde{\SSS}_{i}, \UUU_{i}^{\star} + \Delta\UUU_{i}, \ZZZ_{i}^{\star} + \Delta\ZZZ_i) \\
        + J_{\NNN_i} (\tilde{\YYY}_{\NNN_i}, \tilde{\SSS}_{\NNN_i}, \UUU_{\NNN_i}^{\star} + \Delta\UUU_{\NNN_i}, \ZZZ_{\NNN_i}^{\star} + \Delta\ZZZ_{\NNN_i})
      \end{multlined} \label{eq:lingpdmpc:obj}\\
      & \text{subject to} \nonumber \\
      & \; \tilde{\mathbf{y}}_{i,k} = \hat{m}_{i,k}^{T} \hat{\textbf{x}}_{i,k},
        \; \tilde{\sigma}_{i,k}^{2} = \hat{\textbf{x}}_{i,t}^{T} \hat{V}_{i,k} \hat{\textbf{x}}_{i,k},\; \text{for all $k\in\III_{t}$} \label{eq:lingpmpc:lingp}\\  
      & \; \norm{\Delta \textbf{x}_{i,k}} \leq \rho_i,\; \text{for all $k\in\III_{t}$} \label{eq:lingpmpc:trustreg} \\
      & \; \{ \tilde{\YYY}_{i}, \tilde{\SSS}_{i}, \UUU_{i}^{\star} + \Delta\UUU_{i}, \ZZZ_{i}^{\star}+ \Delta\ZZZ_i \} \in \CC_i \label{eq:lingpdmpc:local-con} \\
      & \; \{ \tilde{\YYY}_{\NNN_i}, \tilde{\SSS}_{\NNN_i}, \UUU_{\NNN_i}^{\star} + \Delta\UUU_{\NNN_i}, \ZZZ_{\NNN_i}^{\star} + \Delta\ZZZ_{\NNN_i} \} \in \CC_{\NNN_i} \label{eq:lingpdmpc:com-con}
  \end{align}
\end{subequations}
where the constraints hold for all $i \in \VVV$.
The constraints~\eqref{eq:lingpmpc:trustreg} specify the trust region, which is the local neighborhood around the nominal solution in which the \linGP-DMPC subproblem is valid.
By Assumption~\ref{assp:convex-lingp}, the \linGP-DMPC subproblem is convex and therefore can be solved efficiently by a convex solver.
Starting from a nominal solution, the \linGP-SCP algorithm iteratively obtains the convex \linGP-DMPC subproblem around the current nominal solution, solves it, determines whether to accept or reject the new solution and how to adapt the trust region radius.
This algorithm is described in details in \cite{nghiem2019linearized}.


